Segmentation-Based Parametric Painting

We introduce a novel image-to-painting method that facilitates the creation of large-scale, high-fidelity paintings with human-like quality and stylistic variation. To process large images and gain control over the painting process, we introduce a segmentation-based painting process and a dynamic attention map approach inspired by human painting strategies, allowing optimization of brush strokes to proceed in batches over different image regions, thereby capturing both large-scale structure and fine details, while also allowing stylistic control over detail. Our optimized batch processing and patch-based loss framework enable efficient handling of large canvases, ensuring our painted outputs are both aesthetically compelling and functionally superior as compared to previous methods, as confirmed by rigorous evaluations. Code available at: https://github.com/manuelladron/semantic\_based\_painting.git

==> figures/fig_tex/abstractions_v2.tex <==
\begin{figure}[t]
\centering
% Row 3
\begin{subfigure}{0.33\linewidth}
\includegraphics[width=\linewidth]{figures/grid_sota/giraffe2_process_text_mask_giraffe_lvl_3.eps}
\caption*{  }
\end{subfigure}\hfill
\begin{subfigure}{0.33\linewidth}
\includegraphics[width=\linewidth]{figures/grid_sota/aw5_composition.eps}
\caption*{Abstract Style}
\end{subfigure}\hfill
\begin{subfigure}{0.33\linewidth}
\includegraphics[width=\linewidth]{figures/grid_sota/combination_isol_masks.eps}
\caption*{  }
\end{subfigure}

\caption{Artistic Abstraction Process. Each piece represents a unique stage of abstraction, capturing the essence of the original in a distinct painterly manner.}
\label{fig:abstractions_v2}
\vspace{-0.5em}
\end{figure}

==> figures/fig_tex/grid_sota_p1.tex <==

\begin{figure*}[htp]
\centering
% Row 1

\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{cvpr24/semantic-based-painting/figures/grid_sota/giraffe_2_div8.png}
\caption*{  }
\end{subfigure}\hfill
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{cvpr24/semantic-based-painting/figures/grid_sota/aw5_sq_1024_div8.png}
\caption*{Learning to Paint (L2P)}
\end{subfigure}\hfill
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{cvpr24/semantic-based-painting/figures/grid_sota/curvy3199_div8.png}
\caption*{  }
\end{subfigure}

% Row 2
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{cvpr24/semantic-based-painting/figures/grid_sota/giraffe2_snp.png}
\caption*{  }
\end{subfigure}\hfill
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{cvpr24/semantic-based-painting/figures/grid_sota/aw5_sq_1024_snp.png}
\caption*{Stylized Neural Painting (SNP)}
\end{subfigure}\hfill
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{cvpr24/semantic-based-painting/figures/grid_sota/curvy3_snp.png}
\caption*{  }
\end{subfigure}

% Row 3
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{cvpr24/semantic-based-painting/figures/grid_sota/giraffe_pt.png}
\caption*{  }
\end{subfigure}\hfill
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{cvpr24/semantic-based-painting/figures/grid_sota/aw5_pt.png}
\caption*{Paint Transformer (PT)}
\end{subfigure}\hfill
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{cvpr24/semantic-based-painting/figures/grid_sota/curvy3_pt.png}
\caption*{  }
\end{subfigure}

% Row 4
% \begin{subfigure}{0.33\textwidth}
% \includegraphics[width=\linewidth]{cvpr24/semantic-based-painting/figures/grid_sota/giraffe2_texture_lvl_3.jpg}
% % % \caption{Seventh image}
% \end{subfigure}\hfill
% \begin{subfigure}{0.33\textwidth}
% \includegraphics[width=\linewidth]{cvpr24/semantic-based-painting/figures/grid_sota/aw5_sq_1024_texture_lvl_3.jpg}
% % \caption{Ours - Realistic}
% \end{subfigure}\hfill
% \begin{subfigure}{0.33\textwidth}
% \includegraphics[width=\linewidth]{cvpr24/semantic-based-painting/figures/grid_sota/curvy3_texture_lvl_3.jpg}
% % \caption{Ninth image}
% \end{subfigure}


% Comparative visualization of paintings generated using four different methods: L2P, SNP, PT, and our method, depicted in the next page. Each column represents a distinct scenario: a giraffe in a natural habitat, a wintry landscape with a tree-lined path, and an architectural structure. We encourage the reader to zoom in to appreciate the details of the paintings. L2p struggles to capture highly detail parts from the trees, while generally giving a good realistic style, although results are blurry and seams are visible. SNP fails to capture small details and it is only able to generate a painterly style. PT struggles capturing fine details like the window framing in the building, and also has a very contrasting use of brushstroke sizes.


\caption{Comparison of four parametric painting techniques—L2P, SNP, PT, and our approach (next page)—across three scenarios: a giraffe in its environment, a snowy landscape, and an architectural structure. Our method's outcomes show improved detail rendition and variability. Note L2P's realistic yet blurry style, SNP's broad painterly effect which struggles to capture fine details (tree branches or windows framing), and PT's inconsistent detail and brushstroke scale. Zoom-in recommended for full appreciation of textural nuances.}
\label{fig:sota_comp_1}
\vspace{-1.5em}
\end{figure*}

% \restoregeometry

==> figures/fig_tex/semantic_process.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=\textwidth]{figures/segmentation_and_maps.eps}
\end{center}
\caption{Semantic-Driven Artistic Rendering. (a) Distinct semantic layers derived from (b) the Semantic map, generated using a segmentation network for refined artistic control. (c) Evolving attention maps across three painting stages focused on mountains, illustrating the adaptive nature of the mapping based on painting progression. (d) Culmination in a painterly representation. (e) Dynamic attention mapping for water regions, highlighting the intricate detailing required where water intersects with rocks and branches.}
\label{fig:semantic_process}
\end{figure*}

==> figures/fig_tex/sota_comp.tex <==
\begin{figure*}[htb!]
\begin{center}
\includegraphics[width=\textwidth]{figures/sota_comp_new_low.eps}
\end{center}
\caption{Comparison with state-of-the-art methods for parametric painting in realistic style. All methods use the official implementation. Reader is encouraged to zoom in to appreciate the difference between paintings. Our method (b) is able to capture the details with higher fidelity than previous methods. L2P (c) produces blurry paintings, Paint Transformer (d) produces highly texturized granular artifacts, and SNP (e) produces very thick strokes that are unable to capture high frequency details.}
\label{fig:sota_comp}
\end{figure*}

==> sec/2_related_work.tex <==
\section{Related Work}
\label{sec:related_work}

Early stroke-based-rendering (SBR) algorithms were mostly procedural, using low-level rules to produce impressionistic effects \cite{Haeberli,Litwinowicz,Hertzmann1998}. Generally, these methods either let the user place strokes \cite{Haeberli}, or strokes are placed on a canvas based on a regular grid \cite{Litwinowicz,Hertzmann1998}. Hertzmann's procedural coarse-to-fine method \cite{Hertzmann1998} models the painting process as a series of layers in which strokes are added based on a regular grid. At each pass, the stroke width is fixed and details are added based on an error threshold. However, this method does not provide any optimization and thus offers limited control over accuracy or style.
We build on this work's layering and detailing method.

While procedural methods successfully generate appealing paintings, they are limited by the lack of stroke placement flexibility. The appeal of optimization-based SBR, however, is that they can encode higher-level artist choices without the need to hard-code where strokes are placed. The first optimization-based painting method \cite{Hertzmann:PBR} generated a effective stroke placement model, however it used inconvenient optimization heuristics. Other early methods such as EM-like packing algorithms were used for non-overlapping stroke primitives \cite{hertzmannSBR,NPRbook}, such as stipples \cite{secord2002weighted} and tile arrangements \cite{kim2002jigsaw}, and a variety of related methods successfully stylize 3D models \cite{meier1996painterly,overcoat}.
% Painterly stylization is a high-dimensional optimization problem, with challenging local minima, and these methods struggle to efficiently achieve economical results for overlapping strokes.
More recently, SBR methods leverage deep networks in which a painting agent is modeled as a neural network and is trained to generate a set of brushstroke parameters that result in a painting version of an input image. The majority of these methods do not use stroke supervision, and deep networks are optimized based on reconstruction losses, which normally are a combination of pixel losses and perceptual losses \cite{johnson2016perceptual,zhang2018perceptual}. All gradient-based approaches use a differentiable rendering engine. Since traditional rendering models are non-differentiable due to the discrete rasterization step, these methods overcome this issue by either using a neural differentiable renderer or a differentiable engine \cite{li2020differentiable}.

Many learning-based SBR use Reinforcement Learning (RL) due to their appeal to model an agent that takes decisions at each painting step \cite{xie2013rl,ganin2018synthesizing, mellor2019unsupervised, huang2019learning, lpaintb, singh2021combining,schaldenbrand}. This agent generates a sequence of strokes based on feedback from a critic network. The learning signal comes in the form of rewards from the critic network, normally trained using adversarial learning \cite{GANs}. Some RL methods focus on accurate depiction \cite{huang2019learning, singh2021combining}. For instance, Huang \textit{et al.}'s method
\cite{huang2019learning} reconstruct images with thousands of tiny strokes, but it is stylistically limited. Schaldenbrand and Oh \cite{schaldenbrand} test variations on this style on a robotic arm. LpaintB \cite{lpaintb} is a combination of RL and self-supervised learning that produces coarser versions of the input image. 

A few other RL methods create more artistic abstractions. One of the first works was SPIRAL \cite{ganin2018synthesizing}, which introduced adversarially-trained actor-critic algorithms, but their results were blurry.
SPIRAL++ \cite{mellor2019unsupervised} presented several improvements, achieving a range of abstracted image styles. However, their method lacked interpretability and control over style and was unable to achieve good reconstructions of the original input. 

There are other methods that do not use RL. For instance, PaintTransformer \cite{Liu_2021_ICCV} uses a CNN-Transformer model and is trained based on predicting foreground strokes given a set of background strokes. Such strokes are synthetically generated and despite not using a dataset, their model shows an excellent generalization capability. However, their paintings are composed by repetitive patterns and often present a stark contrast between stroke sizes. RNN-based methods have also been used to train line drawing and sketching styles that are quite distinct from painting \cite{ha2017neural,kingma2013auto, zheng2018strokenet, mo2021virtualsketching}. We draw inspiration from \cite{mo2021virtualsketching} to model our attention regions.

Aside from neural methods, a few recent work have explored direct differentiable optimization. DiffVG~\cite{li2020differentiable} 
and Stylized Neural Painting (SNP) \cite{Zou_2021_CVPR}
directly optimize the stroke arrangement with gradient-based optimization. SNP generates style variation primarily via style-transfer techniques \cite{Gatys_2016_CVPR, johnson2016perceptual}. 

Among these methods, ``Learning to Paint" \cite{huang2019learning} and SNP \cite{Zou_2021_CVPR} share similar research questions than ours. However, both methods focus on realistic outputs, while we generate a flexible framework that generates a controllable range of paintings, from realism to abstraction. 


==> tables/sota_comp.tex <==
\begin{table}[!h]
\begin{adjustbox}{width=\linewidth, center}
  \centering
  \begin{tabular}{@{}lc@{}c@{}c@{}c@{\hskip.1in}c@{}c@{}c@{}}
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{3}{c}{Model-300S} &\multicolumn{1}{c}{} & \multicolumn{3}{c}{Full Model} \\
    \cmidrule(r){2-4} 
    \cmidrule(r){6-8} 
      & $\mathcal{L}_1\downarrow$ & $\mathcal{L}_{perc} \uparrow$ & N. Strokes & & $\mathcal{L}_1\downarrow$ & $\mathcal{L}_{perc} \uparrow$  & N. Strokes \\
    \midrule
    RL \cite{huang2019learning} & 0.042 & 0.645 & 300 & & 0.040 & 0.814 & 1000\\
    Transformers \cite{Liu_2021_ICCV} & 0.092 & 0.513 & 351 & & 0.068 & 0.678 & 3212 \\
    Optimization \cite{Zou_2021_CVPR} & 0.055 & 0.561 & 300 & & 0.046 & 0.561 & 1000 \\
    Ours$_{D_{LSTM}}$ & 0.048 & 0.658 & 300 & & 0.045 & 0.667 & 1000 \\ 
    Ours$_{D_{LSTM}+FT}$ & \textbf{0.023} & \textbf{0.868} & 300 & & \textbf{0.020} & \textbf{0.899} & 1000 \\ 
    \bottomrule
  \end{tabular}
  \end{adjustbox}
  \caption{ADJUST TABLE Quantitative results on $100$ random sample images drawn from a held-out set on landscapes. We provide metrics on a 300-stroke model (left), and a 1000-stroke model (right). For \cite{Liu_2021_ICCV}, total number of strokes is averaged over the held-out set. We measure $L_1$ loss and perceptual loss using cosine similarity between input image and painting feature maps (higher is better). For a fixed number of strokes, our method achieves a lower perceptual loss than previous methods.}
  \label{tab:sota_landscapes}
\end{table}

==> tables/user_study.tex <==
\begin{table}[h]
\vspace{-1em}
\begin{adjustbox}{width=\linewidth, center}
  \centering
%   \begin{tabular}{@{}lc@{}c@{}c@{}c@{\hskip.1in}c@{}c@{}}
  \begin{tabular}{l c c c c c | c c c c c}
    \toprule
    \multirow{2}{*}{Method} & \multirow{2}{*}{ID} & \multicolumn{2}{c}{Ours} & \multicolumn{2}{c|}{Other} & \multirow{2}{*}{ID} & \multicolumn{2}{c}{Ours} & \multicolumn{2}{c}{Other} \\
    \cmidrule(r){3-4} 
    \cmidrule(r){5-6} 
    \cmidrule(r){8-9}
    \cmidrule(r){10-11}
      & & Votes & Perc. & Votes & Perc. & & Votes & Perc. & Votes & Perc.\\
    \midrule
         \multicolumn{2}{c}{} & \multicolumn{2}{c}{Realistic Paintings} & \multicolumn{2}{c|}{} &  \multicolumn{1}{c}{} & \multicolumn{2}{c}{Visual  Appealing} & \multicolumn{1}{c}{}\\
    \midrule
    L2P & A1 & \textbf{27} & \textbf{67.5\%} & 13 & 32.5\% & B1 & 17 & 42.5\%   &  \textbf{23} & \textbf{57.5}\%  \\
    L2P & A2 & 18 & 45\% &  \textbf{22} & \textbf{55\%} & B2 & 18 & 45\%    & \textbf{22} & \textbf{55\%}  \\
    PT  & A3 & \textbf{37} & \textbf{92.5\%} &  3 & 7.5\% & B3 & \textbf{24} & \textbf{60\%} & 16 & 40\%  \\
    PT  & A4 & \textbf{36} & \textbf{90\%} & 4 & 10\% & B4 & \textbf{31} & \textbf{77.5\%}   & 9 & 22.5\%  \\
    SNP & A5 & \textbf{32} & \textbf{80\%} & 8 & 20\% & B5 & \textbf{33} & \textbf{82.5\%} & 7 & 22.5\%  \\
    SNP & A6 & \textbf{34} & \textbf{85\%} & 6 & 15\%  & B6 & \textbf{26} & \textbf{60\%} & 14 & 40\%  \\
    \midrule
    Total & & \textbf{188} & \textbf{78.3\%} & 52 & 21.6\% & & \textbf{149} & \textbf{62\%} & 91 & 38\% \\
    \bottomrule
  \end{tabular}
  \end{adjustbox}
  \vspace{0.2cm}
  \caption{Qualitative evaluation on user preference: The table's left side contrasts realistic paintings, while the right compares our painterly style to previous methods. Our method was favored by $78.3\%$ for realism and $62\%$ for visual appeal.}
  \label{tab:user_study}
\end{table}
